Teaching Large Language Models to Self-Debug

Large language models (LLMs) have achieved impressive performance on code generation. However, for complex programming tasks, generating the correct solution in one go becomes challenging, thus some prior works have designed program repair approaches to improve code generation performance. In this work, we propose Self-Debugging, which teaches a large language model to debug its predicted program via few-shot demonstrations. In particular, we demonstrate that Self-Debugging can teach the large language model to perform rubber duck debugging; i.e., without any human feedback on the code correctness or error messages, the model is able to identify its mistakes by investigating the execution results and explaining the generated code in natural language. Self-Debugging achieves the state-of-the-art performance on several code generation benchmarks, including the Spider dataset for text-to-SQL generation, TransCoder for C++-to-Python translation, and MBPP for text-to-Python generation. On the Spider benchmark where there are no unit tests to verify the correctness of predictions, Self-Debugging with code explanation consistently improves the baseline by 2-3%, and improves the prediction accuracy on problems of the hardest level by 9%. On TransCoder and MBPP where unit tests are available, Self-Debugging improves the baseline accuracy by up to 12%. Meanwhile, by leveraging feedback messages and reusing failed predictions, Self-Debugging notably improves sample efficiency, and can match or outperform baseline models that generate more than 10x candidate programs.

==> statement.tex <==
\section*{Ethics Statement}

Large language models with strong coding capabilities, combined with \ours{} that allows automated improvement of code quality, may eventually allow for the automation of the development and maintenance of large code bases in addition to the automated explanation of their functionalities and vulnerabilities. Although this can provide great productivity gains, on the flip side, the increasing reliance of model-generated code might also open up new vulnerabilities. Therefore, to deploy any large language model for real-world programming applications, it is crucial to systematically analyze its capabilities and limitations before widely utilizing code generated by the model.

\section*{Reproducibility Statement}

We run all experiments on public benchmarks. We use publicly accessible large language models for evaluation: API access of GPT models is available at \url{https://openai.com/api}, and StarCoder is an open-source LLM~\citep{li2023starcoder}. See Appendices~\ref*{app:spider},~\ref*{app:transcoder} and~\ref*{app:mbpp} for full prompts in experiments on Spider, Transcoder and MBPP benchmarks.
